Video Decoding Energy Reduction Using Temporal-Domain Filtering

In this paper, we study decoding energy reduction opportunities using temporal-domain filtering and subsampling methods. In particular, we study spatiotemporal filtering using a contrast sensitivity function and temporal downscaling, i.e., frame rate reduction. We apply these concepts as a pre-filtering to the video before compression and evaluate the bitrate, the decoding energy, and the visual quality with a dedicated metric targeting temporally down-scaled sequences. We find that decoding energy savings yield 35% when halving the frame rate and that spatiotemporal filtering can lead to up to 5% of additional savings, depending on the content.

==> gfx/ED_curves_v4_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{036}[tc][tc]{ Energy}%
\psfrag{037}[bc][bc]{ GREED}%
\psfrag{039}[tc][tc]{ Energy}%
\psfrag{040}[bc][bc]{ GREED}%
\psfrag{042}[tc][tc]{ Energy}%
\psfrag{043}[bc][bc]{ GREED}%
\psfrag{035}[bc][bc]{ 22}%
\psfrag{038}[bc][bc]{ 17}%
\psfrag{041}[bc][bc]{ 1}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ $0$}%
\psfrag{001}[ct][ct]{ $20$}%
\psfrag{002}[ct][ct]{ $40$}%
\psfrag{003}[ct][ct]{ $60$}%
\psfrag{004}[ct][ct]{ $80$}%
\psfrag{012}[ct][ct]{ $0$}%
\psfrag{013}[ct][ct]{ $5$}%
\psfrag{014}[ct][ct]{ $10$}%
\psfrag{015}[ct][ct]{ $15$}%
\psfrag{023}[ct][ct]{ $0$}%
\psfrag{024}[ct][ct]{ $10$}%
\psfrag{025}[ct][ct]{ $20$}%
\psfrag{026}[ct][ct]{ $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{ $10$}%
\psfrag{006}[rc][rc]{ $15$}%
\psfrag{007}[rc][rc]{ $20$}%
\psfrag{008}[rc][rc]{ $25$}%
\psfrag{009}[rc][rc]{ $30$}%
\psfrag{010}[rc][rc]{ $35$}%
\psfrag{011}[rc][rc]{ $40$}%
\psfrag{016}[rc][rc]{ $14$}%
\psfrag{017}[rc][rc]{ $15$}%
\psfrag{018}[rc][rc]{ $16$}%
\psfrag{019}[rc][rc]{ $17$}%
\psfrag{020}[rc][rc]{ $18$}%
\psfrag{021}[rc][rc]{ $19$}%
\psfrag{022}[rc][rc]{ $20$}%
\psfrag{027}[rc][rc]{ $15$}%
\psfrag{028}[rc][rc]{ $20$}%
\psfrag{029}[rc][rc]{ $25$}%
\psfrag{030}[rc][rc]{ $30$}%
\psfrag{031}[rc][rc]{ $35$}%
\psfrag{032}[rc][rc]{ $40$}%
\psfrag{033}[rc][rc]{ $45$}%
\psfrag{034}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/ED_performance_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{013}[tc][tc]{ Energy in [J]}%
\psfrag{014}[bc][bc]{ VMAF Score}%
\psfrag{000}[ct][ct]{ $4$}%
\psfrag{001}[ct][ct]{ $5$}%
\psfrag{002}[ct][ct]{ $6$}%
\psfrag{003}[ct][ct]{ $7$}%
\psfrag{004}[ct][ct]{ $8$}%
\psfrag{005}[ct][ct]{ $9$}%
\psfrag{006}[rc][rc]{ $70$}%
\psfrag{007}[rc][rc]{ $75$}%
\psfrag{008}[rc][rc]{ $80$}%
\psfrag{009}[rc][rc]{ $85$}%
\psfrag{010}[rc][rc]{ $90$}%
\psfrag{011}[rc][rc]{ $95$}%
\psfrag{012}[rc][rc]{ $100$}%
%
%% </ytick>

==> gfx/RD_curves_v4_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{027}[tc][tc]{ Energy}%
\psfrag{028}[bc][bc]{ GREED}%
\psfrag{030}[tc][tc]{ Energy}%
\psfrag{031}[bc][bc]{ GREED}%
\psfrag{033}[tc][tc]{ Energy}%
\psfrag{034}[bc][bc]{ GREED}%
\psfrag{026}[bc][bc]{ 22}%
\psfrag{029}[bc][bc]{ 17}%
\psfrag{032}[bc][bc]{ 1}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ 10^{6}}%
\psfrag{008}[ct][ct]{ 10^{6}}%
\psfrag{016}[ct][ct]{ 10^{5}}%
\psfrag{017}[ct][ct]{ 10^{6}}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{001}[rc][rc]{ $10$}%
\psfrag{002}[rc][rc]{ $15$}%
\psfrag{003}[rc][rc]{ $20$}%
\psfrag{004}[rc][rc]{ $25$}%
\psfrag{005}[rc][rc]{ $30$}%
\psfrag{006}[rc][rc]{ $35$}%
\psfrag{007}[rc][rc]{ $40$}%
\psfrag{009}[rc][rc]{ $14$}%
\psfrag{010}[rc][rc]{ $15$}%
\psfrag{011}[rc][rc]{ $16$}%
\psfrag{012}[rc][rc]{ $17$}%
\psfrag{013}[rc][rc]{ $18$}%
\psfrag{014}[rc][rc]{ $19$}%
\psfrag{015}[rc][rc]{ $20$}%
\psfrag{018}[rc][rc]{ $15$}%
\psfrag{019}[rc][rc]{ $20$}%
\psfrag{020}[rc][rc]{ $25$}%
\psfrag{021}[rc][rc]{ $30$}%
\psfrag{022}[rc][rc]{ $35$}%
\psfrag{023}[rc][rc]{ $40$}%
\psfrag{024}[rc][rc]{ $45$}%
\psfrag{025}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/RD_performance_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{019}[tc][tc]{ Rate}%
\psfrag{020}[bc][bc]{ VMAF}%
\psfrag{021}[tc][tc]{ Rate}%
\psfrag{022}[bc][bc]{ PSNR}%
\psfrag{000}[tc][tc]{ $\times10^{5}$}%
\psfrag{010}[tc][tc]{ $\times10^{5}$}%
\psfrag{001}[ct][ct]{ $0$}%
\psfrag{002}[ct][ct]{ $0.5$}%
\psfrag{003}[ct][ct]{ $1$}%
\psfrag{004}[ct][ct]{ $1.5$}%
\psfrag{005}[ct][ct]{ $2$}%
\psfrag{011}[ct][ct]{ $0$}%
\psfrag{012}[ct][ct]{ $0.5$}%
\psfrag{013}[ct][ct]{ $1$}%
\psfrag{014}[ct][ct]{ $1.5$}%
\psfrag{015}[ct][ct]{ $2$}%
\psfrag{006}[rc][rc]{ $70$}%
\psfrag{007}[rc][rc]{ $80$}%
\psfrag{008}[rc][rc]{ $90$}%
\psfrag{009}[rc][rc]{ $100$}%
\psfrag{016}[rc][rc]{ $35$}%
\psfrag{017}[rc][rc]{ $40$}%
\psfrag{018}[rc][rc]{ $45$}%
%
%% </ytick>

==> gfx/STCSF_v2_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{008}[tl][tl]{ Spatial Frequency}%
\psfrag{009}[tr][tr]{ Temp. Frquency}%
\psfrag{010}[bc][bc]{ Contrast}%
\psfrag{000}[ct][ct]{ 10^{0}}%
\psfrag{001}[ct][ct]{ 10^{1}}%
\psfrag{002}[rc][rc]{ 10^{0}}%
\psfrag{003}[rc][rc]{ 10^{1}}%
\psfrag{004}[cr][cr]{ $0$}%
\psfrag{005}[cr][cr]{ $0.2$}%
\psfrag{006}[cr][cr]{ $0.4$}%
\psfrag{007}[cr][cr]{ $0.6$}%
%
%% </ztick>

==> gfx/ded_performance_3_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
\psfrag{036}[tc][tc]{ Energy}%
\psfrag{037}[bc][bc]{ GREED}%
\psfrag{039}[tc][tc]{ Energy}%
\psfrag{040}[bc][bc]{ GREED}%
\psfrag{042}[tc][tc]{ Energy}%
\psfrag{043}[bc][bc]{ GREED}%
\psfrag{035}[bc][bc]{ 22}%
\psfrag{038}[bc][bc]{ 17}%
\psfrag{041}[bc][bc]{ 1}%
\psfrag{000}[ct][ct]{ $0$}%
\psfrag{001}[ct][ct]{ $20$}%
\psfrag{002}[ct][ct]{ $40$}%
\psfrag{003}[ct][ct]{ $60$}%
\psfrag{004}[ct][ct]{ $80$}%
\psfrag{012}[ct][ct]{ $0$}%
\psfrag{013}[ct][ct]{ $5$}%
\psfrag{014}[ct][ct]{ $10$}%
\psfrag{015}[ct][ct]{ $15$}%
\psfrag{023}[ct][ct]{ $0$}%
\psfrag{024}[ct][ct]{ $10$}%
\psfrag{025}[ct][ct]{ $20$}%
\psfrag{026}[ct][ct]{ $30$}%
\psfrag{005}[rc][rc]{ $10$}%
\psfrag{006}[rc][rc]{ $15$}%
\psfrag{007}[rc][rc]{ $20$}%
\psfrag{008}[rc][rc]{ $25$}%
\psfrag{009}[rc][rc]{ $30$}%
\psfrag{010}[rc][rc]{ $35$}%
\psfrag{011}[rc][rc]{ $40$}%
\psfrag{016}[rc][rc]{ $14$}%
\psfrag{017}[rc][rc]{ $15$}%
\psfrag{018}[rc][rc]{ $16$}%
\psfrag{019}[rc][rc]{ $17$}%
\psfrag{020}[rc][rc]{ $18$}%
\psfrag{021}[rc][rc]{ $19$}%
\psfrag{022}[rc][rc]{ $20$}%
\psfrag{027}[rc][rc]{ $15$}%
\psfrag{028}[rc][rc]{ $20$}%
\psfrag{029}[rc][rc]{ $25$}%
\psfrag{030}[rc][rc]{ $30$}%
\psfrag{031}[rc][rc]{ $35$}%
\psfrag{032}[rc][rc]{ $40$}%
\psfrag{033}[rc][rc]{ $45$}%
\psfrag{034}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/greed_energy_dec_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
\psfrag{026}[tc][tc]{ Energy}%
\psfrag{027}[bc][bc]{ GREED}%
\psfrag{029}[tc][tc]{ Energy}%
\psfrag{030}[bc][bc]{ GREED}%
\psfrag{032}[tc][tc]{ Energy}%
\psfrag{033}[bc][bc]{ GREED}%
\psfrag{025}[bc][bc]{ 17}%
\psfrag{028}[bc][bc]{ 3}%
\psfrag{031}[bc][bc]{ 1}%
\psfrag{000}[ct][ct]{ $0$}%
\psfrag{001}[ct][ct]{ $5$}%
\psfrag{002}[ct][ct]{ $10$}%
\psfrag{003}[ct][ct]{ $15$}%
\psfrag{008}[ct][ct]{ $0$}%
\psfrag{009}[ct][ct]{ $10$}%
\psfrag{010}[ct][ct]{ $20$}%
\psfrag{016}[ct][ct]{ $0$}%
\psfrag{017}[ct][ct]{ $10$}%
\psfrag{018}[ct][ct]{ $20$}%
\psfrag{019}[ct][ct]{ $30$}%
\psfrag{004}[rc][rc]{ $14$}%
\psfrag{005}[rc][rc]{ $16$}%
\psfrag{006}[rc][rc]{ $18$}%
\psfrag{007}[rc][rc]{ $20$}%
\psfrag{011}[rc][rc]{ $15$}%
\psfrag{012}[rc][rc]{ $20$}%
\psfrag{013}[rc][rc]{ $25$}%
\psfrag{014}[rc][rc]{ $30$}%
\psfrag{015}[rc][rc]{ $35$}%
\psfrag{020}[rc][rc]{ $10$}%
\psfrag{021}[rc][rc]{ $20$}%
\psfrag{022}[rc][rc]{ $30$}%
\psfrag{023}[rc][rc]{ $40$}%
\psfrag{024}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/greed_energy_enc_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{026}[tc][tc]{ Energy}%
\psfrag{027}[bc][bc]{ GREED}%
\psfrag{029}[tc][tc]{ Energy}%
\psfrag{030}[bc][bc]{ GREED}%
\psfrag{032}[tc][tc]{ Energy}%
\psfrag{033}[bc][bc]{ GREED}%
\psfrag{025}[bc][bc]{ 17}%
\psfrag{028}[bc][bc]{ 3}%
\psfrag{031}[bc][bc]{ 1}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ $0$}%
\psfrag{001}[ct][ct]{ $20$}%
\psfrag{002}[ct][ct]{ $40$}%
\psfrag{003}[ct][ct]{ $60$}%
\psfrag{008}[ct][ct]{ $0$}%
\psfrag{009}[ct][ct]{ $100$}%
\psfrag{010}[ct][ct]{ $200$}%
\psfrag{016}[ct][ct]{ $0$}%
\psfrag{017}[ct][ct]{ $100$}%
\psfrag{018}[ct][ct]{ $200$}%
\psfrag{019}[ct][ct]{ $300$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{ $14$}%
\psfrag{005}[rc][rc]{ $16$}%
\psfrag{006}[rc][rc]{ $18$}%
\psfrag{007}[rc][rc]{ $20$}%
\psfrag{011}[rc][rc]{ $15$}%
\psfrag{012}[rc][rc]{ $20$}%
\psfrag{013}[rc][rc]{ $25$}%
\psfrag{014}[rc][rc]{ $30$}%
\psfrag{015}[rc][rc]{ $35$}%
\psfrag{020}[rc][rc]{ $10$}%
\psfrag{021}[rc][rc]{ $20$}%
\psfrag{022}[rc][rc]{ $30$}%
\psfrag{023}[rc][rc]{ $40$}%
\psfrag{024}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/rd_performance_3_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{027}[tc][tc]{ Energy}%
\psfrag{028}[bc][bc]{ GREED}%
\psfrag{030}[tc][tc]{ Energy}%
\psfrag{031}[bc][bc]{ GREED}%
\psfrag{033}[tc][tc]{ Energy}%
\psfrag{034}[bc][bc]{ GREED}%
\psfrag{026}[bc][bc]{ 22}%
\psfrag{029}[bc][bc]{ 17}%
\psfrag{032}[bc][bc]{ 1}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ 10^{6}}%
\psfrag{008}[ct][ct]{ 10^{6}}%
\psfrag{016}[ct][ct]{ 10^{5}}%
\psfrag{017}[ct][ct]{ 10^{6}}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{001}[rc][rc]{ $10$}%
\psfrag{002}[rc][rc]{ $15$}%
\psfrag{003}[rc][rc]{ $20$}%
\psfrag{004}[rc][rc]{ $25$}%
\psfrag{005}[rc][rc]{ $30$}%
\psfrag{006}[rc][rc]{ $35$}%
\psfrag{007}[rc][rc]{ $40$}%
\psfrag{009}[rc][rc]{ $14$}%
\psfrag{010}[rc][rc]{ $15$}%
\psfrag{011}[rc][rc]{ $16$}%
\psfrag{012}[rc][rc]{ $17$}%
\psfrag{013}[rc][rc]{ $18$}%
\psfrag{014}[rc][rc]{ $19$}%
\psfrag{015}[rc][rc]{ $20$}%
\psfrag{018}[rc][rc]{ $15$}%
\psfrag{019}[rc][rc]{ $20$}%
\psfrag{020}[rc][rc]{ $25$}%
\psfrag{021}[rc][rc]{ $30$}%
\psfrag{022}[rc][rc]{ $35$}%
\psfrag{023}[rc][rc]{ $40$}%
\psfrag{024}[rc][rc]{ $45$}%
\psfrag{025}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/share_zeros_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\psfrag{006}[tc][tc]{ Scaling factor}%
\psfrag{007}[bc][bc]{ Share}%
\psfrag{000}[ct][ct]{ $0.01$}%
\psfrag{001}[ct][ct]{ $0.1$}%
\psfrag{002}[ct][ct]{ $1$}%
\psfrag{003}[rc][rc]{ $40$}%
\psfrag{004}[rc][rc]{ $60$}%
\psfrag{005}[rc][rc]{ $80$}%
%
%% </ytick>

==> gfx/x05_fig_qualityDeg_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
\psfrag{025}[tc][tc]{ Scaling}%
\psfrag{026}[bc][bc]{ VMAF}%
\psfrag{027}[tc][tc]{ Scaling}%
\psfrag{028}[bc][bc]{ PSNR}%
\psfrag{000}[ct][ct]{ $1$}%
\psfrag{001}[ct][ct]{ $2$}%
\psfrag{002}[ct][ct]{ $3$}%
\psfrag{003}[ct][ct]{ $4$}%
\psfrag{004}[ct][ct]{ $5$}%
\psfrag{005}[ct][ct]{ $6$}%
\psfrag{012}[ct][ct]{ $1$}%
\psfrag{013}[ct][ct]{ $2$}%
\psfrag{014}[ct][ct]{ $3$}%
\psfrag{015}[ct][ct]{ $4$}%
\psfrag{016}[ct][ct]{ $5$}%
\psfrag{017}[ct][ct]{ $6$}%
\psfrag{006}[rc][rc]{ $90$}%
\psfrag{007}[rc][rc]{ $92$}%
\psfrag{008}[rc][rc]{ $94$}%
\psfrag{009}[rc][rc]{ $96$}%
\psfrag{010}[rc][rc]{ $98$}%
\psfrag{011}[rc][rc]{ $100$}%
\psfrag{018}[rc][rc]{ $35$}%
\psfrag{019}[rc][rc]{ $40$}%
\psfrag{020}[rc][rc]{ $45$}%
\psfrag{021}[rc][rc]{ $50$}%
\psfrag{022}[rc][rc]{ $55$}%
\psfrag{023}[rc][rc]{ $60$}%
\psfrag{024}[rc][rc]{ $65$}%
%
%% </ytick>
